Selective, Interpretable, and Motion Consistent Privacy Attribute Obfuscation for Action Recognition

Concerns for the privacy of individuals captured in public imagery have led to privacy-preserving action recognition. Existing approaches often suffer from issues arising through obfuscation being applied globally and a lack of interpretability. Global obfuscation hides privacy sensitive regions, but also contextual regions important for action recognition. Lack of interpretability erodes trust in these new technologies. We highlight the limitations of current paradigms and propose a solution: Human selected privacy templates that yield interpretability by design, an obfuscation scheme that selectively hides attributes and also induces temporal consistency, which is important in action recognition. Our approach is architecture agnostic and directly modifies input imagery, while existing approaches generally require architecture training. Our approach offers more flexibility, as no retraining is required, and outperforms alternatives on three widely used datasets.

==> teaserfiguresold/teaser2.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
    \centering
    \captionsetup{type=figure}
    \resizebox{\linewidth}{!}{
        \begin{tikzpicture}[spy using outlines={circle, ultra thick, green!40 ,magnification=4.4,size=2.5cm, connect spies}]
            \setlength{\fboxsep}{0pt}
            \begin{scope}
                \node[inner sep=0pt] (one) at (0,-1) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teasershoe.jpg}}};
                \node[inner sep=0pt] (three) at (-1.5, 1.0) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teaserbaby.jpg}}};
                \node[inner sep=0pt] (two) at (2.5, 1.5) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teasersmile.jpg}}};
            \end{scope}

            \node[overlay] at (0.5,4.2) {\huge{Arbitrary Templates}};
            \node[overlay] at (11,4.2) {\huge{Source}};
            \node[overlay] at (11,-0.8) {\huge{Saliency Map}};
            \node[overlay] at (21,4.2) {\huge{Optical Flow}};
            \node[overlay] at (21,-0.8) {\huge{\textbf{Motion Consistent Obfuscation}}};
            \node[overlay] at (29.2,4.2) {\huge{Task}};


            \draw (5.4,-5) -- (5.4,4);
            \draw (26.5,-5) -- (26.5,4);

            \node[inner sep=0pt] (tmp) at (11,-3) {\filmbox{figures/teaser/sim/0016.png}\filmbox{figures/teaser/sim/0020.png}\filmbox{figures/teaser/sim/0024.png}};
            \node[inner sep=0pt] (tmp) at (11,2) {\filmbox{figures/teaser/rgb/0016.png}\filmbox{figures/teaser/rgb/0020.png}\filmbox{figures/teaser/rgb/0024.png}};
            \node[inner sep=0pt] (tmp) at (21,-3) {\filmbox{figures/teaser/obf/0016.png}\filmbox{figures/teaser/obf/0020.png}\filmbox{figures/teaser/obf/0024.png}};  
            \node[inner sep=0pt] (tmp) at (21,2) {\filmbox{figures/teaser/flow/0016.png}\filmbox{figures/teaser/flow/0020.png}\filmbox{figures/teaser/flow/0024.png}};  


            \node[inner sep=0pt] (map) at (29.2,-0.65) {\includegraphics[width=4.8cm]{figures/teaser/teaser.pdf}};


            \spy on (-2.4, 1.1) in node at (-3.2,-4); % Baby
            % \spy on (-0.33, -2.45) in node at (-1,-4); % SHoe
            % \spy on (0.2, -1.6) in node at (-1,-4); % knee his right
            \spy on (-0.27, -1.5) in node at (-1,-4); % knee his left
            \spy on (2.45, 1.75) in node at (1.2,-4); % Nose
            \spy on (2.8, 2) in node at (3.4,-4); % Eye
            % \spy on (2.75, -1.22) in node at (2,-2);
        \end{tikzpicture}
    }
    \captionof{figure}{\textbf{Our goal is to hide privacy attributes without action recognition performance dropping - no retraining required!}\\  
    Arbitrary images, and patches from these images can be used to build a semantic library of features. A saliency map of the templates can be composed, tailored to the specific usecase. A naive masking of these features could be used to hide the privacy attributes, but does not preserve the dynamics important for action recognition. We propose to apply motion conistent noise according to the saliency map, preserving dynamics information, and therefore retaining temporal features crucial for action recognition.}    \label{fig:teaser}
\end{center}%
}]

==> teaserfiguresold/teaser3.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
    \centering
    \captionsetup{type=figure}
    \resizebox{\linewidth}{!}{
        \begin{tikzpicture}[spy using outlines={circle, ultra thick, green!40 ,magnification=4.4,size=2.5cm, connect spies}]
            \setlength{\fboxsep}{0pt}
            \begin{scope}
                \node[inner sep=0pt] (one) at (0,-1) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teasershoe.jpg}}};
                \node[inner sep=0pt] (three) at (-1.5, 1.0) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teaserbaby.jpg}}};
                \node[inner sep=0pt] (two) at (2.5, 1.5) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teasersmile.jpg}}};
            \end{scope}

            \node[overlay] at (0.5,4.2) {\huge{Arbitrary Templates}};
            \node[overlay] at (11,4.2) {\huge{Source}};
            \node[overlay] at (11,-0.8) {\huge{Saliency Map}};
            \node[overlay] at (21,4.2) {\huge{Optical Flow}};
            \node[overlay] at (21,-0.8) {\huge{\textbf{Motion Consistent Obfuscation}}};
            % \node[overlay] at (29.2,4.2) {\huge{Task}};


            % \draw (5.4,-5) -- (5.4,4);
            % \draw (26.5,-5) -- (26.5,4);

            \node[inner sep=0pt] (tmp) at (11,-3) {\filmbox{figures/teaser/sim/0016.png}\filmbox{figures/teaser/sim/0020.png}\filmbox{figures/teaser/sim/0024.png}};
            \node[inner sep=0pt] (tmp) at (11,2) {\filmbox{figures/teaser/rgb/0016.png}\filmbox{figures/teaser/rgb/0020.png}\filmbox{figures/teaser/rgb/0024.png}};
            \node[inner sep=0pt] (tmp) at (21,-3) {\filmbox{figures/teaser/obf/0016.png}\filmbox{figures/teaser/obf/0020.png}\filmbox{figures/teaser/obf/0024.png}};  
            \node[inner sep=0pt] (tmp) at (21,2) {\filmbox{figures/teaser/flow/0016.png}\filmbox{figures/teaser/flow/0020.png}\filmbox{figures/teaser/flow/0024.png}};  


            % \node[inner sep=0pt] (map) at (29.2,-0.65) {\includegraphics[width=4.8cm]{figures/teaser/teaser.pdf}};


            \spy on (-2.4, 1.1) in node at (-3.2,-4); % Baby
            % \spy on (-0.33, -2.45) in node at (-1,-4); % SHoe
            % \spy on (0.2, -1.6) in node at (-1,-4); % knee his right
            \spy on (-0.27, -1.5) in node at (-1,-4); % knee his left
            \spy on (2.45, 1.75) in node at (1.2,-4); % Nose
            \spy on (2.8, 2) in node at (3.4,-4); % Eye
            % \spy on (2.75, -1.22) in node at (2,-2);
        \end{tikzpicture}
    }
    \captionof{figure}{\textbf{Our goal is to hide privacy attributes without action recognition performance dropping - no retraining required!}\\  
    Arbitrary images, and patches from these images can be used to build a semantic library of features. A saliency map of the templates can be composed, tailored to the specific usecase. A naive masking of these features could be used to hide the privacy attributes, but does not preserve the dynamics important for action recognition. We propose to apply motion conistent noise according to the saliency map, preserving dynamics information, and therefore retaining temporal features crucial for action recognition.}    \label{fig:teaser}
\end{center}%
}]

==> teaserfiguresold/teaser4.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
    \centering
    \captionsetup{type=figure}
    \resizebox{\linewidth}{!}{
        \begin{tikzpicture}[spy using outlines={circle, ultra thick, green!40 ,magnification=4.4,size=2.5cm, connect spies}]
            \setlength{\fboxsep}{0pt}
            \begin{scope}
                \node[inner sep=0pt] (one) at (0,-1) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teasershoe.jpg}}};
                \node[inner sep=0pt] (three) at (-1.5, 1.0) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teaserbaby.jpg}}};
                \node[inner sep=0pt] (two) at (2.5, 1.5) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teasersmile.jpg}}};
            \end{scope}

            % \node[overlay] at (0.5,4.2) {\huge{Arbitrary Templates}};
            % \node[overlay] at (11,4.2) {\huge{Source}};
            % \node[overlay] at (11,-0.8) {\huge{Saliency Map}};
            % \node[overlay] at (21,4.2) {\huge{Optical Flow}};
            % \node[overlay] at (21,-0.8) {\huge{\textbf{Motion Consistent Obfuscation}}};
            % \node[overlay] at (29.2,4.2) {\huge{Task}};


            \node[overlay] at (0.5,4.2) {\huge{Arbitrary Templates}};
            \node[overlay] at (9.5,4.2) {\huge{Source}};
            \node[overlay] at (9.5,-0.8) {\huge{Saliency Map}};
            \node[overlay] at (19.5,4.2) {\huge{Optical Flow}};
            \node[overlay] at (21,-0.8) {\huge{\textbf{Motion Consistent Obfuscation}}};
            % \node[overlay] at (29.2,4.2) {\huge{Task}};

            % \draw (5.4,-5) -- (5.4,4);
            % \draw (26.5,-5) -- (26.5,4);

            \node[inner sep=0pt] (tmp) at (11,-3) {\filmbox{figures/teaser/sim/0016.png}\filmbox{figures/teaser/sim/0020.png}\phantom{\filmbox{figures/teaser/sim/0024.png}}};
            \node[inner sep=0pt] (tmp) at (11,2) {\filmbox{figures/teaser/rgb/0016.png}\filmbox{figures/teaser/rgb/0020.png}\phantom{\filmbox{figures/teaser/rgb/0024.png}}};
            \node[inner sep=0pt] (tmp) at (21,-3) {\filmbox{figures/teaser/obf/0016.png}\filmbox{figures/teaser/obf/0020.png}\phantom{\filmbox{figures/teaser/obf/0024.png}}};   
            \node[inner sep=0pt] (tmp) at (21,2) {\filmbox{figures/teaser/flow/0016.png}\filmbox{figures/teaser/flow/0020.png}\phantom{\filmbox{figures/teaser/flow/0024.png}}};   


            % \node[inner sep=0pt] (map) at (29.2,-0.65) {\includegraphics[width=4.8cm]{figures/teaser/teaser.pdf}};


            \spy on (-2.4, 1.1) in node at (-3.2,-4); % Baby
            % \spy on (-0.33, -2.45) in node at (-1,-4); % SHoe
            % \spy on (0.2, -1.6) in node at (-1,-4); % knee his right
            \spy on (-0.27, -1.5) in node at (-1,-4); % knee his left
            \spy on (2.45, 1.75) in node at (1.2,-4); % Nose
            \spy on (2.8, 2) in node at (3.4,-4); % Eye

            \spy [blue, circle, magnification=4, size=3cm] on (12.1, 1.8) in node at (14.1, 2);
            \spy [blue, circle, magnification=4, size=3cm] on (12.1, -3.2) in node at (14.1, -3);

            \spy [blue, circle, magnification=4, size=3cm] on (22.1, 1.8) in node at (24.1, 2);
            \spy [blue, circle, magnification=4, size=3cm] on (22.1, -3.2) in node at (24.1, -3);

            % \spy on (2.75, -1.22) in node at (2,-2);
        \end{tikzpicture}
    }
    \captionof{figure}{\textbf{Our goal is to hide privacy attributes without action recognition performance dropping - no retraining required!}\\  
    Arbitrary images, and patches from these images can be used to build a semantic library of features. A saliency map of the templates can be composed, tailored to the specific usecase. A naive masking of these features could be used to hide the privacy attributes, but does not preserve the dynamics important for action recognition. We propose to apply motion conistent noise according to the saliency map, preserving dynamics information, and therefore retaining temporal features crucial for action recognition.}    \label{fig:teaser}
\end{center}%
}]

==> teaserfiguresold/teasernew.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
    \centering
    \captionsetup{type=figure}
    \resizebox{1.0\linewidth}{!}{
        \begin{tikzpicture}[spy using outlines={circle, ultra thick, green!40 ,magnification=4.4,size=2.5cm, connect spies}]
            \setlength{\fboxsep}{0pt}
            \begin{scope}
                \node[inner sep=0pt] (one) at (0,-1) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teasershoe.jpg}}};
                \node[inner sep=0pt] (three) at (-1.5, 1.0) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teaserbaby.jpg}}};
                \node[inner sep=0pt] (two) at (2.5, 1.5) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teasersmile.jpg}}};
            \end{scope}

            % \node[overlay] at (0.5,4.2) {\huge{Arbitrary Templates}};
            % \node[overlay] at (11,4.2) {\huge{Source}};
            % \node[overlay] at (11,-0.8) {\huge{Saliency Map}};
            % \node[overlay] at (21,4.2) {\huge{Optical Flow}};
            % \node[overlay] at (21,-0.8) {\huge{\textbf{Motion Consistent Obfuscation}}};
            % \node[overlay] at (29.2,4.2) {\huge{Task}};


            \node[overlay] at (0.5,4.2) {\huge{Arbitrary Templates}};
            \node[overlay] at (10.5,4.2) {\huge{Source}};
            \node[overlay] at (10.5,-0.8) {\huge{Saliency Map}};
            \node[overlay] at (22.5,4.2) {\huge{Optical Flow}};
            % \node[overlay] at (23,-0.8) {\huge{\textbf{Motion Consistent Obfuscation}}};
            \node[overlay] at (22.5,-0.8) {\huge{\textbf{Obfuscation}}};
            % \node[overlay] at (29.2,4.2) {\huge{Task}};
            \node[overlay] at (22.5,-5.2) {\Large{\textit{Temporally Consistent!}}};

            \draw (5.9,-5) -- (5.9,4);
            % \draw (26.5,-5) -- (26.5,4);

            \node[inner sep=0pt] (tmp) at (12,-3) {\filmbox{figures/teaser/sim/0016.png}\filmbox{figures/teaser/sim/0020.png}\phantom{\filmbox{figures/teaser/sim/0024.png}}};
            \node[inner sep=0pt] (tmp) at (12,2) {\filmbox{figures/teaser/rgb/0016.png}\filmbox{figures/teaser/rgb/0020.png}\phantom{\filmbox{figures/teaser/rgb/0024.png}}};
            \node[inner sep=0pt] (tmp) at (24,-3) {\filmbox{figures/teaser/obf/0016.png}\filmbox{figures/teaser/obf/0020.png}\phantom{\filmbox{figures/teaser/obf/0024.png}}};   
            \node[inner sep=0pt] (tmp) at (24,2) {\filmbox{figures/teaser/flow/0016.png}\filmbox{figures/teaser/flow/0020.png}\phantom{\filmbox{figures/teaser/flow/0024.png}}};   


            % \node[inner sep=0pt] (map) at (29.2,-0.65) {\includegraphics[width=4.8cm]{figures/teaser/teaser.pdf}};


            \spy on (-2.4, 1.1) in node at (-3.2,-4); % Baby
            % \spy on (-0.33, -2.45) in node at (-1,-4); % SHoe
            % \spy on (0.2, -1.6) in node at (-1,-4); % knee his right
            \spy on (-0.27, -1.5) in node at (-1,-4); % knee his left
            \spy on (2.45, 1.75) in node at (1.2,-4); % Nose
            \spy on (2.8, 2) in node at (3.4,-4); % Eye

            \spy [blue, circle, magnification=4, size=4.0cm] on (13.1, 1.8) in node at (15.8, 3.5);
            \spy [blue, circle, magnification=4, size=4.0cm] on (13.1, -3.2) in node at (15.8, -1.5);

            \spy [blue, circle, magnification=4, size=4.0cm] on (25.1, 1.8) in node at (27.8, 3.5);
            \spy [blue, circle, magnification=4, size=4.0cm] on (25.1, -3.2) in node at (27.8, -1.5);

            % \spy on (2.75, -1.22) in node at (2,-2);
        \end{tikzpicture}
    }
    \captionof{figure}{\textbf{Our goal is to hide privacy attributes without action recognition performance dropping - no retraining required!}\\  
    Arbitrary images, and patches from these images can be used to build a semantic library of features. A saliency map of the templates can be composed, tailored to the specific usecase. A naive masking of these features could be used to hide the privacy attributes, but does not preserve the dynamics important for action recognition. We propose to apply motion conistent noise according to the saliency map, preserving dynamics information, and therefore retaining temporal features crucial for action recognition.}
    \label{fig:teaser}
\end{center}%
}]

==> teaserfiguresold/teaserold.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
    \centering
    \captionsetup{type=figure}
    \resizebox{\linewidth}{!}{
        \begin{tikzpicture}[spy using outlines={circle, ultra thick, green!40 ,magnification=4.4,size=2.5cm, connect spies}]
            \setlength{\fboxsep}{0pt}
            \begin{scope}
                \node[inner sep=0pt] (one) at (0,-1) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teasershoe.jpg}}};
                \node[inner sep=0pt] (three) at (-1.5, 1.0) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teaserbaby.jpg}}};
                \node[inner sep=0pt] (two) at (2.5, 1.5) {\fbox{\includegraphics[width=.25\textwidth]{figures/teaser/teasersmile.jpg}}};
            \end{scope}

            % \node[overlay] at (0.5,4.2) {\huge{Arbitrary Templates}};
            % \node[overlay] at (11,4.2) {\huge{Source}};
            % \node[overlay] at (11,-0.8) {\huge{Saliency Map}};
            % \node[overlay] at (21,4.2) {\huge{Optical Flow}};
            % \node[overlay] at (21,-0.8) {\huge{\textbf{Motion Consistent Obfuscation}}};
            % \node[overlay] at (29.2,4.2) {\huge{Task}};


            \node[overlay] at (0.5,4.2) {\huge{Arbitrary Templates}};
            \node[overlay] at (9.5,4.2) {\huge{Source}};
            \node[overlay] at (9.5,-0.8) {\huge{Saliency Map}};
            \node[overlay] at (19.5,4.2) {\huge{Optical Flow}};
            \node[overlay] at (21,-0.8) {\huge{\textbf{Motion Consistent Obfuscation}}};
            \node[overlay] at (29.2,4.2) {\huge{Task}};

            \draw (5.4,-5) -- (5.4,4);
            \draw (26.5,-5) -- (26.5,4);

            \node[inner sep=0pt] (tmp) at (11,-3) {\filmbox{figures/teaser/sim/0016.png}\filmbox{figures/teaser/sim/0020.png}\phantom{\filmbox{figures/teaser/sim/0024.png}}};
            \node[inner sep=0pt] (tmp) at (11,2) {\filmbox{figures/teaser/rgb/0016.png}\filmbox{figures/teaser/rgb/0020.png}\phantom{\filmbox{figures/teaser/rgb/0024.png}}};
            \node[inner sep=0pt] (tmp) at (21,-3) {\filmbox{figures/teaser/obf/0016.png}\filmbox{figures/teaser/obf/0020.png}\phantom{\filmbox{figures/teaser/obf/0024.png}}};   
            \node[inner sep=0pt] (tmp) at (21,2) {\filmbox{figures/teaser/flow/0016.png}\filmbox{figures/teaser/flow/0020.png}\phantom{\filmbox{figures/teaser/flow/0024.png}}};   


            \node[inner sep=0pt] (map) at (29.2,-0.65) {\includegraphics[width=4.8cm]{figures/teaser/teaser.pdf}};


            \spy on (-2.4, 1.1) in node at (-3.2,-4); % Baby
            % \spy on (-0.33, -2.45) in node at (-1,-4); % SHoe
            % \spy on (0.2, -1.6) in node at (-1,-4); % knee his right
            \spy on (-0.27, -1.5) in node at (-1,-4); % knee his left
            \spy on (2.45, 1.75) in node at (1.2,-4); % Nose
            \spy on (2.8, 2) in node at (3.4,-4); % Eye

            \spy [blue, circle, magnification=4, size=3cm] on (12.1, 1.8) in node at (14.1, 2);
            \spy [blue, circle, magnification=4, size=3cm] on (12.1, -3.2) in node at (14.1, -3);

            \spy [blue, circle, magnification=4, size=3cm] on (22.1, 1.8) in node at (24.1, 2);
            \spy [blue, circle, magnification=4, size=3cm] on (22.1, -3.2) in node at (24.1, -3);

            % \spy on (2.75, -1.22) in node at (2,-2);
        \end{tikzpicture}
    }
    \captionof{figure}{\textbf{Our goal is to hide privacy attributes without action recognition performance dropping - no retraining required!}\\  
    Arbitrary images, and patches from these images can be used to build a semantic library of features. A saliency map of the templates can be composed, tailored to the specific usecase. A naive masking of these features could be used to hide the privacy attributes, but does not preserve the dynamics important for action recognition. We propose to apply motion conistent noise according to the saliency map, preserving dynamics information, and therefore retaining temporal features crucial for action recognition.}    \label{fig:teaser}
\end{center}%
}]
